On the Effectiveness of Image Manipulation Detection in the Age of Social Media

Image manipulation detection algorithms designed to identify local anomalies often rely on the manipulated regions being ``sufficiently'' different from the rest of the non-tampered regions in the image. However, such anomalies might not be easily identifiable in high-quality manipulations, and their use is often based on the assumption that certain image phenomena are associated with the use of specific editing tools. This makes the task of manipulation detection hard in and of itself, with state-of-the-art detectors only being able to detect a limited number of manipulation types. More importantly, in cases where the anomaly assumption does not hold, the detection of false positives in otherwise non-manipulated images becomes a serious problem. To understand the current state of manipulation detection, we present an in-depth analysis of deep learning-based and learning-free methods, assessing their performance on different benchmark datasets containing tampered and non-tampered samples. We provide a comprehensive study of their suitability for detecting different manipulations as well as their robustness when presented with non-tampered data. Furthermore, we propose a novel deep learning-based pre-processing technique that accentuates the anomalies present in manipulated regions to make them more identifiable by a variety of manipulation detection methods. To this end, we introduce an anomaly enhancement loss that, when used with a residual architecture, improves the performance of different detection algorithms with a minimal introduction of false positives on the non-manipulated data. Lastly, we introduce an open-source manipulation detection toolkit comprising a number of standard detection algorithms.

==> tables/GliderEval_AUC.tex <==
\begin{center}\begin{tabular}{|r|l|l|}
\hline
\textbf{Algorithm} & \textbf{AUC (\%)}   & \textbf{AEN AUC (\%)}                                      \\ \hline \hline
\textbf{BLK~\cite{li2009passive}} &	00.98 $\pm$ 00.23 & \textbf{00.98 $\pm$ 00.23	($\uparrow$ 	1.13E-05)} \\ \hline
\textbf{DCT~\cite{ye2007detecting}} &	01.55 $\pm$ 01.71 & \textbf{03.76 $\pm$ 10.34	($\uparrow$ 	02.21)} \\ \hline
\textbf{ELA~\cite{ela_krawetz2007}} &	03.17 $\pm$ 01.69 & 02.61 $\pm$ 01.01	($\downarrow$ 	00.56) \\ \hline \hline
\textbf{CFA1~\cite{Dirik2009ImageTD}} &	08.60 $\pm$ 16.46 & 01.77 $\pm$ 06.06	($\downarrow$ 	06.83) \\ \hline
\textbf{CFA2~\cite{Ferrara2012ImageFL}} &	01.21 $\pm$ 00.68 & 01.05 $\pm$ 00.41	($\downarrow$ 	00.16) \\ \hline \hline
\textbf{NOI1~\cite{MAHDIAN20091497}} &	01.71 $\pm$ 01.46 & 01.11 $\pm$ 00.50	($\downarrow$ 	00.61) \\ \hline
\textbf{NOI2~\cite{lyu2014exposing}} &	43.95 $\pm$ 09.41 & \textbf{45.45 $\pm$ 06.52	($\uparrow$ 	01.50)} \\ \hline
\textbf{NOI4~\cite{noi4_wagner2015}} &	26.63 $\pm$ 08.40 & 24.21 $\pm$ 08.44	($\downarrow$ 	02.42) \\ \hline \hline
\textbf{Mantra-Net~\cite{wu2019mantra}} &	03.03 $\pm$ 01.71 & \textbf{10.45 $\pm$ 05.06	($\uparrow$ 	07.42)} \\ \hline
\textbf{RGBN~\cite{zhou2018learning}}                            & 06.42 $\pm$	11.35 & \textbf{12.16 $\pm$	13.11	 ($\uparrow$ 05.74)}\\ \hline

\end{tabular}
\end{center}

==> tables/GliderEval_GWL1.tex <==
\begin{center}\begin{tabular}{|r|l|l|}
\hline
\textbf{Algorithm} & \textbf{GWL1 (\%)}   & \textbf{AEN GWL1 (\%)}                                      \\ \hline \hline
\textbf{BLK~\cite{li2009passive}}       & 28.87 $\pm$ 07.99     & \textbf{24.45 $\pm$ 07.87 ($\downarrow$ 04.41)} \\ \hline
\textbf{DCT~\cite{ye2007detecting}}       & 48.46 $\pm$ 07.12 & \textbf{44.17 $\pm$ 11.33 ($\downarrow$ 04.29)}             \\ \hline
\textbf{ELA~\cite{ela_krawetz2007}}       & 09.68 $\pm$ 02.22 & 10.82 $\pm$ 05.03 ($\uparrow$ 01.13)            \\ \hline \hline
\textbf{CFA1~\cite{Dirik2009ImageTD}}      & 64.43 $\pm$ 25.40 & 76.03 $\pm$ 10.49 ($\uparrow$ 11.60)            \\ \hline
\textbf{CFA2~\cite{Ferrara2012ImageFL}}      & 36.40 $\pm$ 11.96 & \textbf{28.48 $\pm$ 08.56 ($\downarrow$ 07.92)}  \\ \hline \hline
\textbf{NOI1~\cite{MAHDIAN20091497}}      & 13.41 $\pm$ 05.99 & 14.78 $\pm$ 06.53 ($\uparrow$ 01.37)            \\ \hline
\textbf{NOI2~\cite{lyu2014exposing}}      & 00.36 $\pm$ 01.25   & \textbf{00.18 $\pm$ 00.50 ($\downarrow$ 00.18)}  \\ \hline
\textbf{NOI4~\cite{noi4_wagner2015}}      & 01.23 $\pm$ 01.53  & \textbf{00.85 $\pm$ 00.83 ($\downarrow$ 00.38)}  \\ \hline \hline
\textbf{Mantra-Net~\cite{wu2019mantra}}  & 07.66 $\pm$ 02.63	& \textbf{06.40 $\pm$ 01.34 ($\downarrow$ 01.26)} \\ \hline
\textbf{RGBN~\cite{zhou2018learning}}                            & 87.16 $\pm$	22.70 & \textbf{75.67 $\pm$	26.22	 ($\downarrow$11.48)}\\ \hline

\end{tabular}
\end{center}


==> tables/Glider_Baseline.tex <==
\begin{center}\begin{tabular}{|r|r|r|}
\hline
\textbf{Algorithm} & \textbf{GWL1 (\%)}   & \textbf{AUC (\%)}                                      \\ \hline \hline
\textbf{BLK~\cite{li2009passive}}	& 28.87 $\pm$ 07.99	& 0.98 $\pm$ 00.23	\\ \hline
\textbf{DCT~\cite{ye2007detecting}}	& 48.46 $\pm$ 07.12	& 01.55 $\pm$ 01.71	\\ \hline
\textbf{ELA~\cite{ela_krawetz2007}}	& 09.68 $\pm$ 02.22	& 03.17 $\pm$ 01.69	\\ \hline \hline
\textbf{CFA1~\cite{Dirik2009ImageTD}}	& 64.43 $\pm$ 25.40	& 08.60 $\pm$ 16.46	\\ \hline
\textbf{CFA2~\cite{Ferrara2012ImageFL}}	& 36.40 $\pm$ 11.96	& 01.21 $\pm$ 00.68	\\ \hline \hline
\textbf{NOI1~\cite{MAHDIAN20091497}}	& 13.41 $\pm$ 05.99	& 01.71 $\pm$ 01.46	\\ \hline
\textbf{NOI2~\cite{lyu2014exposing}}	& \textbf{0.36 $\pm$ 01.25}	& \textbf{43.95 $\pm$ 09.41}	\\ \hline
\textbf{NOI4~\cite{noi4_wagner2015}}	& 01.23 $\pm$ 01.53 & 26.63 $\pm$ 08.40	\\ \hline \hline
\textbf{Mantra-Net~\cite{wu2019mantra}}	& 07.66 $\pm$ 02.63	& 03.03 $\pm$ 01.71	\\ \hline
\textbf{RGBN~\cite{zhou2018learning}} & 87.16 $\pm$	22.70 &	06.42 $\pm$	11.35 \\ \hline

\end{tabular}
\end{center}

==> tables/INet_Baseline.tex <==
\begin{center}\begin{tabular}{|r|r|r|}
\hline
\textbf{Algorithm} & \textbf{GWL1 (\%)}   & \textbf{AUC (\%)}                                      \\ \hline \hline
\textbf{BLK~\cite{li2009passive}}	& 31.52 $\pm$ 08.56	& 02.52 $\pm$ 01.22	\\ \hline
\textbf{DCT~\cite{ye2007detecting}}	& 45.44 $\pm$ 12.13	& 03.84 $\pm$ 04.28	\\ \hline
\textbf{ELA~\cite{ela_krawetz2007}}	& 15.43 $\pm$ 08.05	& 10.89 $\pm$ 10.70	\\ \hline \hline
\textbf{CFA1~\cite{Dirik2009ImageTD}}	& 57.34 $\pm$ 24.07	& 10.20 $\pm$ 16.16	\\ \hline
\textbf{CFA2~\cite{Ferrara2012ImageFL}}	& 33.01 $\pm$ 10.11	& 02.91 $\pm$ 02.22	\\ \hline \hline
\textbf{NOI1~\cite{MAHDIAN20091497}}	& 14.81 $\pm$ 08.25	& 04.14 $\pm$ 04.42	\\ \hline
\textbf{NOI2~\cite{lyu2014exposing}}	& 05.41 $\pm$ 05.18	& \textbf{20.18 $\pm$ 14.99}	\\ \hline
\textbf{NOI4~\cite{noi4_wagner2015}}	& \textbf{02.46 $\pm$ 01.75}	& 19.94 $\pm$ 08.66	\\ \hline \hline
\textbf{Mantra-Net~\cite{wu2019mantra}}	& 05.39 $\pm$ 02.29	& 06.94 $\pm$ 04.40	\\ \hline
\textbf{RGBN~\cite{zhou2018learning}} & 56.37 $\pm$	31.41	& 21.82 $\pm$	15.71 \\ \hline

\end{tabular}
\end{center}

==> tables/Imagenette_SMAPE.tex <==
\begin{center}
\begin{tabular}{|r|l|l|}
\hline
\textbf{Algorithm}   & \textbf{Baseline} & \textbf{AEN}             \\ \hline \hline
\textbf{BLK~\cite{li2009passive}}       & $99.91 \pm 0.84$\%    & $99.93 \pm 0.55$\% ($\uparrow$ 0.02\%)  \\ \hline
\textbf{DCT~\cite{ye2007detecting}}       & $95.87 \pm 10.16$\%   & $97.59 \pm 8.29$\% ($\uparrow$ 1.73\%)   \\ \hline
\textbf{ELA~\cite{ela_krawetz2007}}       & $82.24 \pm 22.15$\%   & $96.90 \pm 4.86$\% ($\uparrow$ 14.66\%)   \\ \hline \hline
\textbf{CFA1~\cite{Dirik2009ImageTD}}      & $83.01 \pm 34.48$\%   & $86.41 \pm 31.80$\% ($\uparrow$ 3.40\%)   \\ \hline
\textbf{CFA2~\cite{Ferrara2012ImageFL}}      & $98.26 \pm 5.57$\%    & $98.80 \pm 4.47$\% ($\uparrow$ 0.53\%)    \\ \hline \hline
\textbf{NOI1~\cite{MAHDIAN20091497}}      & $95.12 \pm 10.39$\%   & $97.48 \pm 7.20$\% ($\uparrow$ 2.36\%)   \\ \hline
\textbf{NOI2~\cite{lyu2014exposing}}      & $61.09 \pm 31.75$\%   & \textbf{$47.32 \pm 28.94$\% ($\downarrow$ 13.78\%)} \\ \hline
\textbf{NOI4~\cite{noi4_wagner2015}}      & $63.25 \pm 18.03$\%   & $66.64 \pm 18.19$\% ($\uparrow$ 3.38\%)  \\ \hline \hline
\textbf{Mantra-Net~\cite{wu2019mantra}} & $90.72 \pm 9.34$\%    & \textbf{$76.67 \pm 14.50$\% ($\downarrow$ 14.05\%)} \\ \hline
\end{tabular}
\end{center}

==> tables/MDev_Baseline.tex <==
\begin{center}
\begin{tabular}{|r|r|r|}
\hline
\textbf{Algorithm} & \textbf{GWL1 (\%)}   & \textbf{AUC (\%)}                                      \\ \hline \hline
\textbf{BLK~\cite{li2009passive}}       & 31.23 $\pm$ 10.29	& 59.11 $\pm$ 28.57 \\ \hline
\textbf{DCT~\cite{ye2007detecting}}       & 35.58 $\pm$ 15.94	& 59.20 $\pm$ 26.80  \\ \hline
\textbf{ELA~\cite{ela_krawetz2007}}       & 11.95 $\pm$ 09.86	& 56.22 $\pm$ 19.76  \\ \hline \hline
\textbf{CFA1~\cite{Dirik2009ImageTD}}      & 55.56 $\pm$ 27.77	& 55.54 $\pm$ 23.17 \\ \hline
\textbf{CFA2~\cite{Ferrara2012ImageFL}}      & 28.39 $\pm$ 11.49	& 53.11 $\pm$ 24.88 \\ \hline \hline
\textbf{NOI1~\cite{MAHDIAN20091497}}      & 15.24 $\pm$ 11.68 & 56.52 $\pm$ 33.81 \\ \hline
\textbf{NOI2~\cite{lyu2014exposing}}      & \textbf{05.52 $\pm$ 10.50}	& 54.37 $\pm$ 18.34 \\ \hline
\textbf{NOI4~\cite{noi4_wagner2015}}      & 05.97 $\pm$ 10.27	& 49.30 $\pm$ 17.44  \\ \hline \hline
\textbf{Mantra-Net~\cite{wu2019mantra}}  & 10.16 $\pm$ 09.18	& \textbf{62.98 $\pm$ 23.53} \\ \hline
\textbf{RGBN~\cite{zhou2018learning}} & 24.01 $\pm$ 29.35	& 52.67 $\pm$ 16.43 \\ \hline


\end{tabular}
\end{center}

==> tables/MEval_Baseline.tex <==
\begin{center}
\begin{tabular}{|r|r|r|}
\hline
\textbf{Algorithm} & \textbf{GWL1 (\%)}   & \textbf{AUC (\%)}                                     \\ \hline \hline
\textbf{BLK~\cite{li2009passive}}	& 43.42 $\pm$ 30.75	& 58.12 $\pm$ 25.14	\\ \hline
\textbf{DCT~\cite{ye2007detecting}}	& 42.98 $\pm$ 36.03	& 54.19 $\pm$ 24.45	\\ \hline
\textbf{ELA~\cite{ela_krawetz2007}}	& 41.54 $\pm$ 36.58	& 53.93 $\pm$ 16.60	\\ \hline \hline
\textbf{CFA1~\cite{Dirik2009ImageTD}}	& 41.14 $\pm$ 33.50	& 54.88 $\pm$ 22.98	\\ \hline
\textbf{CFA2~\cite{Ferrara2012ImageFL}}	& 27.05 $\pm$ 25.90	& 56.12 $\pm$ 24.80	\\ \hline \hline
\textbf{NOI1~\cite{MAHDIAN20091497}}	& 39.43 $\pm$ 36.02	& 54.87 $\pm$ 29.53	\\ \hline
\textbf{NOI2~\cite{lyu2014exposing}}	& \textbf{10.86 $\pm$ 17.09}	& 52.19 $\pm$ 11.59	\\ \hline
\textbf{NOI4~\cite{noi4_wagner2015}}	& 15.34 $\pm$ 17.72	& 47.94 $\pm$ 13.61	\\ \hline \hline
\textbf{Mantra-Net~\cite{wu2019mantra}}	& 19.08 $\pm$ 25.96	& \textbf{67.92 $\pm$ 22.40}	\\ \hline
\textbf{RGBN~\cite{zhou2018learning}} & 24.11 $\pm$	25.54	& 57.61 $\pm$	17.00 \\ \hline

\end{tabular}
\end{center}

==> tables/MFCDev_AUC.tex <==
\begin{center}
\begin{tabular}{|r|l|l|}
\hline
\textbf{Algorithm} & \textbf{AUC (\%)}   & \textbf{AEN AUC (\%)}                                     \\ \hline \hline
\textbf{BLK~\cite{li2009passive}}        & 59.11 $\pm$ 28.57 & \textbf{59.33 $\pm$ 28.40 ($\uparrow$ 00.22)}  \\ \hline
\textbf{DCT~\cite{ye2007detecting}}        & 59.20 $\pm$ 26.80   & 49.12 $\pm$ 19.65 ($\downarrow$ 10.08)       \\ \hline
\textbf{ELA~\cite{ela_krawetz2007}}        & 56.22 $\pm$ 19.76 & \textbf{57.10 $\pm$ 20.49 ($\uparrow$ 00.88)}  \\ \hline \hline
\textbf{CFA1~\cite{Dirik2009ImageTD}}       & 55.54 $\pm$ 23.17 & \textbf{58.22 $\pm$ 21.85 ($\uparrow$ 02.69)} \\ \hline
\textbf{CFA2~\cite{Ferrara2012ImageFL}}       & 53.11 $\pm$ 24.88 & 42.79 $\pm$ 22.21 ($\downarrow$ 10.32)       \\ \hline \hline
\textbf{NOI1~\cite{MAHDIAN20091497}}       & 56.52 $\pm$ 33.81 & \textbf{59.14 $\pm$ 32.32 ($\uparrow$ 02.62)} \\ \hline
\textbf{NOI2~\cite{lyu2014exposing}}       & 54.37 $\pm$ 18.34 & 52.73 $\pm$ 16.64 ($\downarrow$ 01.64)        \\ \hline
\textbf{NOI4~\cite{noi4_wagner2015}}       & 49.30 $\pm$ 17.44  & \textbf{52.25 $\pm$ 18.23 ($\uparrow$ 02.95)} \\ \hline \hline
\textbf{Mantra-Net~\cite{wu2019mantra}}  & 62.98 $\pm$ 23.53 & 61.27 $\pm$ 20.45 ($\downarrow$ 01.71) \\ \hline
\textbf{RGBN~\cite{zhou2018learning}}                            & 52.67 $\pm$ 16.43 & \textbf{57.61 $\pm$	20.97 ($\uparrow$ 04.93)}\\ \hline


\end{tabular}
\end{center}

==> tables/MFCDev_BWL1.tex <==
\begin{center}
\begin{tabular}{|r|l|l|}
\hline
\textbf{Algorithm}  & \textbf{Baseline}   & \textbf{BWL1}                               \\ \hline \hline
\textbf{BLK~\cite{li2009passive}}        & 36.64 $\pm$ 33.57\% & \textbf{34.36 $\pm$ 33.81\% ($\downarrow$ 2.28\%)} \\ \hline
\textbf{DCT~\cite{ye2007detecting}}        & 38.43 $\pm$ 34.70\% & 53.32 $\pm$ 35.83\% ($\uparrow$ 14.89\%)           \\ \hline
\textbf{ELA~\cite{ela_krawetz2007}}        & 22.35 $\pm$ 24.67\% & 25.40 $\pm$ 27.02\% ($\uparrow$ 3.05\%)             \\ \hline
\textbf{CFA1~\cite{Dirik2009ImageTD}}       & 37.79 $\pm$ 36.50\% & 42.04 $\pm$ 31.73\% ($\uparrow$ 4.24\%)            \\ \hline
\textbf{CFA2~\cite{Ferrara2012ImageFL}}       & 46.90 $\pm$ 37.17\% & 58.99 $\pm$ 37.76\% ($\uparrow$ 12.09\%)           \\ \hline
\textbf{NOI1~\cite{MAHDIAN20091497}}       & 34.31 $\pm$ 36.07\% & 34.53 $\pm$ 35.32\% ($\uparrow$ 0.23\%)            \\ \hline
\textbf{NOI2~\cite{lyu2014exposing}}       & 6.66 $\pm$ 11.65\%  & \textbf{6.41 $\pm$ 10.55\% ($\downarrow$ 0.25\%)}  \\ \hline
\textbf{NOI4~\cite{noi4_wagner2015}}       & 9.80 $\pm$ 13.51\%  & 11.93 $\pm$ 14.31\% ($\uparrow$ 2.13\%)            \\ \hline
\textbf{Mantra-Net~\cite{wu2019mantra}}  & 27.3 $\pm$ 31.27\%	& 23.6 $\pm$ 23.03\% ($\downarrow$ 3.7\%) \\ \hline
\end{tabular}
\end{center}

==> tables/MFCDev_EER.tex <==
\begin{center}
\begin{tabular}{|r|l|l|}
\hline
\textbf{Algorithm} & \textbf{Baseline}   & \textbf{EER}                                       \\ \hline \hline
\textbf{BLK~\cite{li2009passive}}       & 40.41 $\pm$ 22.5\%  & \textbf{39.92 $\pm$ 22.70\% ($\downarrow$ 0.49\%)}  \\ \hline
\textbf{CFA1~\cite{Dirik2009ImageTD}}      & 43.93 $\pm$ 17.41\% & \textbf{42.24 $\pm$ 15.28\% ($\downarrow$ 1.70\%)}  \\ \hline
\textbf{CFA2~\cite{Ferrara2012ImageFL}}      & 46.18 $\pm$ 18.60\%  & 54.30 $\pm$ 16.68\% ($\uparrow$ 8.12\%)             \\ \hline
\textbf{DCT~\cite{ye2007detecting}}       & 40.99 $\pm$ 20.06\% & 49.43 $\pm$ 13.68\% ($\uparrow$ 8.43\%)            \\ \hline
\textbf{ELA~\cite{ela_krawetz2007}}       & 43.57 $\pm$ 12.75\% & \textbf{42.80 $\pm$ 13.37\% ($\downarrow$ 0.77\%)}  \\ \hline
\textbf{NOI1~\cite{MAHDIAN20091497}}      & 42.11 $\pm$ 28.21\% & 39.77 $\pm$ 25.98\% ($\downarrow$ 2.34\%)          \\ \hline
\textbf{NOI2~\cite{lyu2014exposing}}      & 44.03 $\pm$ 13.41\% & 45.49 $\pm$ 12.00\% ($\uparrow$ 1.45\%)               \\ \hline
\textbf{NOI4~\cite{noi4_wagner2015}}      & 49.3 $\pm$ 11.78\%  & \textbf{46.47 $\pm$ 12.00\% ($\downarrow$ 2.83\%)}    \\ \hline
\textbf{Mantra-Net~\cite{wu2019mantra}}  & 38.01 $\pm$ 17.31\%	& 39.59 $\pm$ 13.89\% ($\uparrow$1.58\%) \\ \hline
\end{tabular}
\end{center}

==> tables/MFCDev_GWL1.tex <==
\begin{center}
\begin{tabular}{|r|l|l|}
\hline
\textbf{Algorithm} & \textbf{GWL1 (\%)} & \textbf{AEN GWL1 (\%)}                                      \\ \hline \hline
\textbf{BLK~\cite{li2009passive}}       & 31.23 $\pm$ 10.29 & \textbf{28.37 $\pm$ 11.52 ($\downarrow$ 02.86)} \\ \hline
\textbf{DCT~\cite{ye2007detecting}}       & 35.58 $\pm$ 15.94 & 42.65 $\pm$ 15.60 ($\uparrow$ 07.08)             \\ \hline
\textbf{ELA~\cite{ela_krawetz2007}}       & 11.95 $\pm$ 09.86  & 13.38 $\pm$ 09.48 ($\uparrow$ 01.43)             \\ \hline \hline
\textbf{CFA1~\cite{Dirik2009ImageTD}}      & 55.56 $\pm$ 27.77 & 67.76 $\pm$ 19.14 ($\uparrow$ 12.20)            \\ \hline
\textbf{CFA2~\cite{Ferrara2012ImageFL}}      & 28.39 $\pm$ 11.49 & \textbf{27.24 $\pm$ 08.71 ($\downarrow$ 01.15)}  \\ \hline \hline
\textbf{NOI1~\cite{MAHDIAN20091497}}      & 15.24 $\pm$ 11.68 & 16.86 $\pm$ 10.74 ($\uparrow$ 01.63)            \\ \hline
\textbf{NOI2~\cite{lyu2014exposing}}      & 05.52 $\pm$ 10.50   & \textbf{05.37 $\pm$ 10.53 ($\downarrow$ 00.14)}  \\ \hline
\textbf{NOI4~\cite{noi4_wagner2015}}      & 05.97 $\pm$ 10.27  & \textbf{05.86 $\pm$ 10.26 ($\downarrow$ 00.10)}   \\ \hline \hline
\textbf{Mantra-Net~\cite{wu2019mantra}}  & 10.16 $\pm$ 09.18	& 11.73 $\pm$ 08.89 ($\uparrow$ 01.56) \\ \hline
\textbf{RGBN~\cite{zhou2018learning}}                            & 24.01 $\pm$	29.35 & 42.63 $\pm$	26.42	 ($\uparrow$ 18.62)\\ \hline

\end{tabular}
\end{center}

==> tables/MFCEval_AUC.tex <==
\begin{center}
\begin{tabular}{|r|l|l|}
\hline
\textbf{Algorithm} & \textbf{AUC (\%)}   & \textbf{AEN AUC (\%)}                                     \\ \hline \hline
\textbf{BLK~\cite{li2009passive}}       & 58.12 $\pm$ 25.14 & \textbf{59.24 $\pm$ 27.70 ($\uparrow$ 01.12)}  \\ \hline
\textbf{DCT~\cite{ye2007detecting}}       & 54.19 $\pm$ 24.45 & 49.99 $\pm$ 16.05 ($\downarrow$ 04.20)         \\ \hline
\textbf{ELA~\cite{ela_krawetz2007}}       & 53.93 $\pm$ 16.60  & \textbf{54.37 $\pm$ 16.11 ($\uparrow$ 00.44)} \\ \hline \hline
\textbf{CFA1~\cite{Dirik2009ImageTD}}      & 54.88 $\pm$ 22.98 & \textbf{58.20 $\pm$ 19.66 ($\uparrow$ 03.31)}  \\ \hline
\textbf{CFA2~\cite{Ferrara2012ImageFL}}      & 56.12 $\pm$ 24.80  & 51.17 $\pm$ 22.30 ($\downarrow$ 04.95)         \\ \hline \hline
\textbf{NOI1~\cite{MAHDIAN20091497}}      & 54.87 $\pm$ 29.53 & \textbf{59.27 $\pm$ 25.97 ($\uparrow$ 04.39)} \\ \hline
\textbf{NOI2~\cite{lyu2014exposing}}      & 52.19 $\pm$ 11.59 & 51.51 $\pm$ 08.23 ($\downarrow$ 00.69)         \\ \hline
\textbf{NOI4~\cite{noi4_wagner2015}}      & 47.94 $\pm$ 13.61 & \textbf{51.21 $\pm$ 12.98 ($\uparrow$ 03.27)} \\ \hline \hline
\textbf{Mantra-Net~\cite{wu2019mantra}}  & 67.92 $\pm$ 22.40	& 60.50 $\pm$ 20.48 ($\downarrow$ 07.41) \\ \hline
\textbf{RGBN~\cite{zhou2018learning}}                            & 57.61 $\pm$ 17.00 & \textbf{65.64 $\pm$	20.07 ($\uparrow$ 08.03)}\\ \hline
\end{tabular}
\end{center}

==> tables/MFCEval_BWL1.tex <==
\begin{center}
\begin{tabular}{|r|l|l|}
\hline
\textbf{Algorithm} & \textbf{Baseline}   & \textbf{BWL1}                               \\ \hline \hline
\textbf{BLK~\cite{li2009passive}}       & 43.42 $\pm$ 30.75\% & \textbf{38.95 $\pm$ 33.62\% ($\downarrow$ 4.47\%)} \\ \hline
\textbf{CFA1~\cite{Dirik2009ImageTD}}      & 42.98 $\pm$ 36.03\% & \textbf{42.89 $\pm$ 31.17\% ($\downarrow$ 0.09\%)} \\ \hline
\textbf{CFA2~\cite{Ferrara2012ImageFL}}      & 41.54 $\pm$ 36.58\% & 51.17 $\pm$ 36.69\% ($\uparrow$ 9.63\%)            \\ \hline
\textbf{DCT~\cite{ye2007detecting}}       & 41.14 $\pm$ 33.5\%  & 53.22 $\pm$ 34.47\% ($\uparrow$ 12.09\%)           \\ \hline
\textbf{ELA~\cite{ela_krawetz2007}}       & 27.05 $\pm$ 25.9\%  & 28.54 $\pm$ 25.76\% ($\uparrow$ 1.49\%)            \\ \hline
\textbf{NOI1~\cite{MAHDIAN20091497}}      & 39.43 $\pm$ 36.02\% & 40.27 $\pm$ 33.03\% ($\uparrow$ 0.84\%)            \\ \hline
\textbf{NOI2~\cite{lyu2014exposing}}      & 10.86 $\pm$ 17.09\% & \textbf{10.22 $\pm$ 16.88\% ($\downarrow$ 0.65\%)} \\ \hline
\textbf{NOI4~\cite{noi4_wagner2015}}      & 15.34 $\pm$ 17.72\% & 19.47 $\pm$ 20.21\% ($\uparrow$ 4.13\%)            \\ \hline
\textbf{Mantra-Net~\cite{wu2019mantra}}  & 19.08 $\pm$ 25.96\%	& 28.54 $\pm$ 25.69\% ($\uparrow$ 9.47\%) \\ \hline
\end{tabular}
\end{center}

==> tables/MFCEval_EER.tex <==
\begin{center}
\begin{tabular}{|r|l|l|}
\hline
\textbf{Algorithm} & \textbf{Baseline}   & \textbf{EER}                                       \\ \hline \hline
\textbf{BLK~\cite{li2009passive}}       & 42.82 $\pm$ 21.67\% & \textbf{41.85 $\pm$ 24.03\% ($\downarrow$ 0.98\%)} \\ \hline
\textbf{CFA1~\cite{Dirik2009ImageTD}}      & 45.95 $\pm$ 19.49\% & \textbf{43.49 $\pm$ 15.99\% ($\downarrow$ 2.46\%)} \\ \hline
\textbf{CFA2~\cite{Ferrara2012ImageFL}}      & 44.68 $\pm$ 21.21\% & 49.28 $\pm$ 18.42\% ($\uparrow$ 4.60\%)             \\ \hline
\textbf{DCT~\cite{ye2007detecting}}       & 46.57 $\pm$ 20.14\% & 49.93 $\pm$ 12.86\% ($\uparrow$ 3.36\%)            \\ \hline
\textbf{ELA~\cite{ela_krawetz2007}}       & 46.51 $\pm$ 13.13\% & \textbf{46.05 $\pm$ 12.70\% ($\downarrow$ 0.46\%)}  \\ \hline
\textbf{NOI1~\cite{MAHDIAN20091497}}      & 44.67 $\pm$ 25.36\% & \textbf{41.50 $\pm$ 22.02\% ($\downarrow$ 3.17\%)}  \\ \hline
\textbf{NOI2~\cite{lyu2014exposing}}      & 47.70 $\pm$ 9.93\%  & 48.27 $\pm$ 7.27\% ($\uparrow$ 0.57\%)             \\ \hline
\textbf{NOI4~\cite{noi4_wagner2015}}      & 51.72 $\pm$ 11.58\% & \textbf{48.79 $\pm$ 10.72\% ($\downarrow$ 2.94\%)} \\ \hline
\end{tabular}
\end{center}

==> tables/MFCEval_GWL1.tex <==
\begin{center}\begin{tabular}{|r|l|l|}
\hline
\textbf{Algorithm} & \textbf{GWL1 (\%)}   & \textbf{AEN GWL1 (\%)}                                      \\ \hline \hline
\textbf{BLK~\cite{li2009passive}}       & 32.00 $\pm$ 11.50     & \textbf{30.65 $\pm$ 12.45 ($\downarrow$ 01.35)} \\ \hline
\textbf{DCT~\cite{ye2007detecting}}       & 36.94 $\pm$ 15.81 & 43.61 $\pm$ 14.40 ($\uparrow$ 06.66)             \\ \hline
\textbf{ELA~\cite{ela_krawetz2007}}       & 15.21 $\pm$ 14.75 & 16.66 $\pm$ 14.24 ($\uparrow$ 01.45)            \\ \hline \hline
\textbf{CFA1~\cite{Dirik2009ImageTD}}      & 59.93 $\pm$ 23.04 & 65.91 $\pm$ 20.51 ($\uparrow$ 05.98)            \\ \hline
\textbf{CFA2~\cite{Ferrara2012ImageFL}}      & 29.76 $\pm$ 13.11 & \textbf{29.45 $\pm$ 09.91 ($\downarrow$ 00.31)}  \\ \hline \hline
\textbf{NOI1~\cite{MAHDIAN20091497}}      & 18.83 $\pm$ 15.71 & 19.18 $\pm$ 13.99 ($\uparrow$ 00.35)            \\ \hline
\textbf{NOI2~\cite{lyu2014exposing}}      & 09.30 $\pm$ 16.45   & \textbf{09.13 $\pm$ 16.42 ($\downarrow$ 00.17)}  \\ \hline
\textbf{NOI4~\cite{noi4_wagner2015}}      & 09.84 $\pm$ 16.23  & \textbf{09.68 $\pm$ 16.25 ($\downarrow$ 00.16)}  \\ \hline \hline
\textbf{Mantra-Net~\cite{wu2019mantra}}  & 13.54 $\pm$ 14.44	& 15.35 $\pm$ 13.99 ($\uparrow$ 01.82) \\ \hline
\textbf{RGBN~\cite{zhang2018image}}                            & 24.11 $\pm$	25.54 & 36.49 $\pm$	25.80	 ($\uparrow$ 12.38)\\ \hline
\end{tabular}
\end{center}

